Extending Video Masked Autoencoders to 128 frames

Video understanding has witnessed significant progress with recent video foundation models demonstrating strong performance owing to self-supervised pre-training objectives; Masked Autoencoders (MAE) being the design of choice. Nevertheless, the majority of prior works that leverage MAE pre-training have focused on relatively short video representations (16 / 32 frames in length) largely due to hardware memory and compute limitations that scale poorly with video length due to the dense memory-intensive self-attention decoding. One natural strategy to address these challenges is to subsample tokens to reconstruct during decoding (or decoder masking). In this work, we propose an effective strategy for prioritizing tokens which allows training on longer video sequences (128 frames) and gets better performance than, more typical, random and uniform masking strategies. The core of our approach is an adaptive decoder masking strategy that prioritizes the most important tokens and uses quantized tokens as reconstruction objectives. Our adaptive strategy leverages a powerful MAGVIT-based tokenizer that jointly learns the tokens and their priority. We validate our design choices through exhaustive ablations and observe improved performance of the resulting long-video (128 frames) encoders over short-video (32 frames) counterparts. With our long-video masked autoencoder (LVMAE) strategy, we surpass state-of-the-art on Diving48 by 3.9 points and EPIC-Kitchens-100 verb classification by 2.5 points while relying on a simple core architecture and video-only pre-training (unlike some of the prior works that require millions of labeled video-text pairs or specialized encoders).

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec_conclusion.tex <==
\section{Conclusion}

In this paper we present a relatively simple but highly effective adaptive masking strategy for video MAE pre-training that allows us to pre-train on long videos (128 frames). Our approach is based on a novel MAGVIT-based tokenization strategy that also learns importance of tokens. Further, we are the first, to our knowledge, to show that long-video MAE pre-training is not only possible but leads to better encodings. Using our approach we are able to achieve state-of-the-art downstream performance, despite using a simple architecture and video only pre-training.   
%is useful in leading to SoTA performance. Our strong performance is in spite of the fact that we use a simple architecture and video only pre-training. 

==> sec_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Long video understanding has witnessed growing interest with various aspects of the problem having been explored by recent works \cite{wu2021towards,mangalam2024egoschema}. This includes incorporating (i) efficient attention mechanisms \cite{islam2022long,wang2023selective} to reduce memory footprint which enables training over longer video sequences, (ii) designing memory modules \cite{balavzevic2024memory,wu2022memvit,ryoo2023token} to reason over context from the past, and (iii) approaching the problem from video-language domain by proposing benchmarks \cite{mangalam2024egoschema,islam2024video} and architectural choices which effectively leverage the interplay between the modalities \cite{papalampidi2023simple,zhang2023simple,sun2022long,islam2024video,tan2024koala}.


At the same time, there has been a drive in pushing the frontiers of vision foundation models \cite{radford2021learning,wang2022internvideo, wang2024internvideo2,zhao2024videoprism,fang2023eva} which focuses on \textit{scaling} pre-training and multi-modal alignment on various vision tasks. The success and effectiveness of such approaches is largely underpinned by the use of vanilla ViT encoder \cite{dosovitskiy2020image} and pre-training with masked video modelling and/or contrastive learning objectives on unlabelled videos and video-language data respectively \cite{zhao2024videoprism,wang2024internvideo2}.

However, the existing long-video understanding approaches fall short on (i) \textit{scalability} of architectural design choices, where for example, State-Space based architectures require substituting attention layers with S4 layer \cite{gu2021efficiently}, or selective fine-tuning of additional memory modules \cite{feichtenhofer2022masked}, 
and (ii) modelling videos as first citizen (or \textit{video-first} approach), where, in the context of video-language tasks, LLoVi \cite{zhang2023simple} shows a greater role of language encoder in achieving improved performance on language-based long-video QA benchmarks \cite{mangalam2024egoschema}. A recent work, LongViViT \cite{papalampidi2023simple} explored strategies to scale video-language contrastive pre-training over long-video sequences by adapting ViT encoder from short-video (16 frames) to long-video (128 frames) by randomly masking out $75\%$ of the input video tokens.

Most existing video models can encode only a few frames (16-32) at a time [cites]. This limits their ability to understand actions and events spanning longer time horizons. While current models are limited to low-level tasks like atomic action recognition, long-context video models could understand longer actions (like complex diving routines), whole activities consisting of a sequence of actions and eventually entire story arcs. Existing work has worked around the short context issue by segmenting longer input video into short chunks and feeding them into the video model sequentially. Inference results from these chunks are then joined using late fusion. For example, "multi-crop" evaluations simply average-pool predictions over all chunks.

Given the effectiveness of scale and downstream performance of masked video modelling, in this work, we ask the question: \textit{Is there an effective strategy to scale masked video modelling to long-videos?}

Masked Autoencoders (MAE) has emerged as a simple and effective approach to masked video modelling \cite{feichtenhofer2022masked,wang2023videomae}. It involves encoding a small fraction of visible / unmasked tokens (=$10\%$) of an input video, and decoding the remaining masked tokens (=$90\%$) using dense space-time attention decoder blocks. However, for longer video sequences, reconstructing all the masked tokens at the decoding stage quickly leads to out-of-memory (OOM) due to quadratic complexity of Transformers (feasible only for less than $64$ frames). The memory requirement can be partially addressed by reducing the batch size used during pre-training, but this comes at the cost of total training time, rendering the setup prohibitively time-consuming and infeasible.

Prior attempts to reduce memory bottleneck in MAE takes the form of either (i) sub-sampling a subset of ``informative" tokens instead of using the entire set of spatio-temporal tokens (EVEREST \cite{hwang2023everest}), or (ii) reconstructing a subset of tokens at the decoding stage or \textit{decoder masking} (VideoMAEv2 \cite{wang2023videomae}). The resulting gains have been shown to reduce training time and hardware requirement \cite{hwang2023everest}, and can be reinvested to scale model size \cite{wang2023videomae}. However, scaling the input video along the temporal dimension has received little-to-no attention besides scaling input frames to a higher spatial resolution [CITE].



In this work, we build on \textit{dual masking} \cite{wang2023videomae} which performs masking at both the encoding and decoding stages. In particular, we use a token-saliency scheme (such as motion) and propose an \textbf{adaptive dual masking strategy} for videos in the MAE setup. The core idea is that the token-saliency scheme establishes a rank-order of video tokens, which is then used to sub-sample higher-ranking tokens for decoding (\nitesh{drop}or forward-masking). 

% This has two-fold consequences: first, sub-sampling tokens to be reconstructed at decoder stage lowers the memory requirement and enables modelling long-videos in MAE, and second, reconstructing / decoding higher-salient (forward-masking) tokens using lower-salient encoder tokens (inverse-masking) poses a meaningful reconstruction objective, which enables competitive performance in low-budget scenarios.



Our contributions are as follows:
\begin{enumerate}
    \item Given a low-token budget, our adaptive dual masking strategy outperforms prior related uniform and motion-based dual masking strategy
    \item The memory savings obtained from low-token budget enables pre-training over long-videos (128 frames), resulting in improved performance
    \item We observe that long-video MAE (128 frames) consistently outperforms short-video MAE (32 frames) measured using downstream fine-tuning performance \nitesh{drop the next phrase}on both short and long-video fine-tuning setup
    \item \nitesh{We demonstrate superior performance on par or exceeding SOTA on conventional action classification benchmarks including Epic-Kitchens-100, Diving-48 and SSv2 using standard ViT encoders and just one temporal crop}
    % We experiment with conventional action classification benchmarks including Epic-Kitchens-100 and Diving-48, and show improved performance of long-vides
\end{enumerate}



==> sec_related_work.tex <==
\section{Related work}
\label{sec:related_work}

\vspace{0.1in}
\noindent
\textbf{Motion in Video MAE}.
In MAE, attempts to identify and attribute relevance to video tokens involved in motion compared to static background, has seen growing interests \cite{huang2023mgmae,fan2023motion} since motion is fundamental to understanding videos. In particular, MGMAE \cite{huang2023mgmae} and MGM \cite{fan2023motion} show that an informed encoder masking based on motion-cues at \nitesh{patch-level??} token-level makes the MAE reconstruction task account for motion, and found faster convergence and improved performance on motion-centric video datasets such as SSv2 \cite{goyal2017something}. Specifically, MGM  \cite{fan2023motion} uses H.264 codec \cite{richardson2002video} to extract \nitesh{patch-level??} token-level motion vectors, and mask out tokens involved in motion during encoding, and MGMAE  \cite{huang2023mgmae} uses online optical flow extractor (RAFT \cite{teed2020raft}), to warp and guide encoder masking using flow.

\nitesh{Unlike these approaches, we do not model motion explicitly, and any apparent motion information in our mask is a product of our data-driven saliency learning scheme.}


% Similar to the above works, our inverse encoder masking aims to mask out tokens involved in motion \cite{fan2023motion}, but differently we don't guide masking across frames and rather form masks on a per-frame basis. Additionally, we propose forward decoder masking as part of our framework to pre-train over long videos, and particularly, place emphasis on strategies that scale to long videos.


\vspace{0.1in}
\noindent
\textbf{Long videos and Masking}.
\nitesh{Masking out tokens during training reduces memory requirement and this fact is exploited in several video understanding works for scaling model size [cite, UMT, VideoPrism, InternVideo]. However, expanding these techniques for long-videos has received limited attention}.  %In the context of long-videos, Masking out tokens during training reduces memory requirement which can be used to train over long videos. 
Recently, LongViViT \cite{papalampidi2023simple} leveraged random masking during contrastive pre-training on video-language tasks, and observed best performance-memory trade-off. Specifically, in order to convert short-video encoder to long-videos, they fine-tune last four layers of ViViT \cite{arnab2021vivit} on long videos (=$128$ frames) along with $75\%$ random masking. Similar to LongViViT \cite{papalampidi2023simple}, we utilize masking to pre-train over long videos.

\nitesh{But differently, first, we focus on masked autoencoder learning instead of contrastive learning for long-videos where decoder masking is prime and second, we pre-train \textit{all the layers} of our model instead of partial freezing in order to capture dense space-time correspondence in long-videos.}



\vspace{0.1in}
\noindent
\textbf{Efficiency as token reduction}.
Sub-sampling salient tokens, based on a learned or an off-the-shelf scheme during training, has been shown to give faster convergence and low-resource requirement \cite{hwang2023everest,zhou2023can,ryoo2021tokenlearner}. In particular, EVEREST \cite{hwang2023everest} attempts to learn what tokens in the spatio-temporal volume of videos are more informative using a heuristic based on distance in feature space (as a proxy for motion), and found that sub-sampling such tokens in MAE setup leads to lower memory consumption and lower resource requirement, while maintaining performance. ObjectViViT \cite{zhou2023can} extracts object bounding boxes using an off-the-shelf object detector, and place emphasis on tokens belonging to objects and found lower token utilization to obtain competitive performance on Epic Kitchens \cite{Damen2022RESCALING} and SSv2 \cite{goyal2017something} benchmarks. Lastly, Token Learner \cite{ryoo2021tokenlearner} observes and correct for token redundancy in higher layers of ViT \cite{dosovitskiy2020image} using learned modules.

Similar to the above approaches, we use token saliency to inform our proposed dual masking setup. Differently, we don't sub-sample tokens, but selectively decode tokens during training phase in a more \textit{generalizable} dual masking setup. \nitesh{EVEREST is the most comparable to our work, but differently, first, our token saliency scheme is learnt separately and independently in a VQVAE setup while EVEREST learns token-saliency during MAE pre-training itself. We argue that the latter approach can bias the method towards selecting \emph{easy} tokens for MAE objective undermining the learning, and second, we predict the salient VQ tokens as targets instead of the salient RGB pixels which offers superior performance.} 


%But differently, first, instead of randomly masking tokens, we use token saliency schemes to inform selection or masking of tokens in a dual masking setup, and second, we pre-train \textit{all the layers} of our model instead of partial freezing in order to capture dense space-time correspondence in videos.%


\vspace{0.1in}
\noindent
\textbf{Long videos and Memory}.
Memory-based approaches \cite{wu2022memvit, balavzevic2024memory} attempt to form a compressed representation of the past activations or memory, which is then incorporated into current window or time step, effectively prolonging the context length over which reasoning and predictions are formed. 
% MeMViT\cite{wu2022memvit}, MC-ViT \cite{balavzevic2024memory} ...
\nitesh{Orthogonal to these works, we expand the local context window of clips during pre-training from 16 to 128 frames, and this can be combined with a memory module to increase the global context window.}



\vspace{0.1in}
\noindent
\textbf{Long-Video Question-Answering (QA)}.
EgoSchema \cite{mangalam2024egoschema} \todo{Expand}. 
\nitesh{This section seems unnecessary.}


% \paragraph{Misc}
% ReST \cite{yang2023relational}, QaEgo4D \cite{barmann2022did}

==> tables/ablations/adaptive.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{\textbf{Why Adaptive?}}
\label{tab:why-adaptive}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|c@{}}
\toprule
MAE Pre-training & Fine-Tuning        \\ \midrule
Target           & Noun-Verb Accuracy \\ \midrule
VQ-VAE           & \todo{TBA}               \\
Ours ()          & \todo{TBA}      \\ \bottomrule
\end{tabular}%
% }
\end{table}

==> tables/ablations/frame_vs_video_level.tex <==

\begin{table}[t]
\centering
\caption{\textbf{Video-level decoder mask outperforms Frame-level}. On EK100, we observe that generating decoder masks where token budget is allocated at video-level is more beneficial than allocating budget at frame-level.}
\label{tab:video-level-vs-frame-level}
% \resizebox{0.85\columnwidth}{!}{%
% \begin{tabular}{@{}ccc|c@{}}
% \toprule
% \multicolumn{3}{c|}{MAE Pre-Training}                                    & Fine-Tuning                    \\ \midrule
% Encoder Masking              & Decoder Masking             & $\rho_d$    & Noun-Verb Accuracy             \\ \midrule
% \multirow{2}{*}{Random Tube} & Frame-level (Flow + Random) & 20\% + 10\% & 39.7                           \\
%                              & Video-level (Flow + Random) & 20\% + 10\% & \textbf{40.7} \\ \bottomrule
% \end{tabular}%

\begin{tabular}{@{}cc|c@{}}
\toprule
\multicolumn{2}{c|}{MAE Pre-training (RGB Target)}  & Fine-Tuning        \\ \midrule
Saliency Scheme             & Mask ratio ($\rho_d$) & Noun-Verb Accuracy \\ \midrule
Frame-level (Flow + Random) & 20\% + 10\%           & 39.7               \\
Video-level (Flow + Random) & 20\% + 10\%           & \textbf{40.7}      \\ \bottomrule
\end{tabular}%
% }
\end{table}

==> tables/ablations/mask-ratios.tex <==

\begin{table}[t]
\centering
\caption{\textbf{Different masking ratios.} We observe (1) }
\label{tab:mask-ratio}

\begin{tabular}{@{}c|c@{}}
\toprule
MAE Pre-training (MAGViT Target) & Fine-Tuning        \\ \midrule
Mask ratio ($\rho_d$)            & Noun-Verb Accuracy \\ \midrule
5\%                         & \todo{TBA}               \\
15\%                      & \todo{TBA}               \\
10\% + 5\%                      & \todo{TBA}      \\
20\% + 10\%                      & \todo{TBA}      \\
\bottomrule
\end{tabular}%
% }
\end{table}

==> tables/long_on_short.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{\textbf{Long video pre-training outperforms on short-videos}. We observe that fine-tuning a long-video (128 frames) MAE pre-trained encoder on short-videos (32 / 64 frames) improves performance compared to fine-tuning their respective short-video MAE pre-trained encoders.}
\label{tab:long-on-short}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccc|cc@{}}
\toprule
                     & \multicolumn{3}{c|}{MAE Pre-Training}                                                & \multicolumn{2}{c}{Fine-Tuning} \\ \midrule
\# Frames           & Encoder Masking               & Decoder Masking                & $\rho_d$                & \# Frames & Noun-Verb Accuracy \\ \midrule
32 & \multirow{2}{*}{Random Tube} & \multirow{2}{*}{None} & \multirow{2}{*}{0\%} & 32  & 40.4 \\ 
64 &  &  &   & 64  & 43.4 \\ \midrule
\multirow{3}{*}{128} & \multirow{3}{*}{Random Tube}  & \multirow{3}{*}{Frame}         & \multirow{3}{*}{50\%} & 32         & \textbf{41.1}               \\
   &             &      &   & 64  & \textbf{44.0} \\
   &             &      &   & 128 & \textbf{44.0} \\ \midrule
\multirow{3}{*}{128} & \multirow{3}{*}{Inverse Flow} & \multirow{3}{*}{Flow + Random} & \multirow{3}{*}{20\% + 10\%} & 32         & \textcolor{red}{todo}                  \\
   &             &      &   & 64  & \textcolor{red}{todo}      \\
   &             &      &   & 128 & \textcolor{red}{todo}      \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/memory-flops.tex <==

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{\textbf{Decoder masking and memory usage in long-video (128 frames) pre-training.} We report memory and FLOPs per-device for a batch size of 1 using different decoder mask ratios with ViT-B encoder.
% % \nitesh{We can have these as plots, 
% % Plot1: Memory vs decoder masking ratio, memory of the encoder is a flat line. Plot2: FLOPS vs decoder masking ratio, FLOPS for the encoder is a flat line. Plot 3 and 4: Same as above for 128 frames. \RG{Agreed}}
% }
% \label{tab:memory-flops}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% \toprule
% Decoder mask ratio ($\rho_d$) & Memory & Flops \\ \midrule
% None (100\%)              & \multicolumn{2}{c}{{\color[HTML]{9B9B9B} out of memory}}      \\
% 50\%                      & \todo{TBA}       & \todo{TBA}      \\
% 15\%                      & \todo{TBA}       & \todo{TBA}      \\ \bottomrule
% \end{tabular}%
% % }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{figure}[]
\centering
\caption{\textbf{Decoder masking and memory usage in long-video (128 frames) pre-training.} We report memory and FLOPs per-device for a batch size of 1 using different decoder mask ratios with ViT-B encoder.
% \nitesh{We can have these as plots, 
% Plot1: Memory vs decoder masking ratio, memory of the encoder is a flat line. Plot2: FLOPS vs decoder masking ratio, FLOPS for the encoder is a flat line. Plot 3 and 4: Same as above for 128 frames. \RG{Agreed}}
}
\label{tab:memory-flops}
% \resizebox{\columnwidth}{!}{%
\vspace{-0.2in}
\includegraphics[width=0.4\textwidth]{tables/figures/flops_and_memory.pdf}
\vspace{-0.3in}
% }
\end{figure}

==> tables/sota_EK.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{\textbf{Comparison to SOTA on EK-100.}. Rows marked with {\color[HTML]{9B9B9B} gray} denote unpublished works. \RG{TAdaFormer seems to be unpublished -- cross-check}}
\label{tab:sota-ek-100}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
Model             & Extra Pre-training Data            & Action & Verb & Noun \\ \midrule
SlowFast~\cite{feichtenhofer2019slowfast}          & K400                 & 38.5   & 65.6 & 50.0 \\
IPL (I3D)~\cite{wang2021interactive}         & K400                 & 41.0   & 68.6 & 51.2 \\
ViViT-L/16x2~\cite{arnab2021vivit}      & IN21K+K400           & 44.0   & 66.4 & 56.8 \\
MoViNet-A5~\cite{kondratyuk2021movinets}        & N/A                  & 44.5   & 69.1 & 55.1 \\
MeMViT-16, 16x4~\cite{wu2022memvit}   & K400                 & 46.2   & 70.6 & 58.5 \\
MeMViT-24, 32x3~\cite{wu2022memvit}   & K600                 & 48.4   & 71.4 & 60.3 \\
Omnivore (Swin-B)~\cite{girdhar2022omnivore} & IN-(21K+1K)+K400+SUN & 49.9   & 69.5 & 61.7 \\
MTV-B~\cite{yan2022multiview}             & IN21K                & 46.7   & 67.8 & 60.5 \\
$\text{MTV-B}_{\uparrow 280^2}$~\cite{yan2022multiview}     & WTS-60M              & 50.5   & 69.9 & 63.9 \\
TAdaFormer-B/16~\cite{huang2023temporally}   & K710                 & 49.1   & 71.0 & 60.5 \\
TAdaFormer-L/16~\cite{huang2023temporally}   & K710                 & 51.8   & 71.7 & 64.1 \\ \midrule
\textit{large vision-language pre-training} \\
LaViLa (TSF-B)~\cite{zhao2023learning}    & WIT + Ego4D          & 46.9   & 69.0 & 58.4 \\
LaViLa (TSF-L)~\cite{zhao2023learning}    & WIT + Ego4D          & 51.0   & 72.0 & 62.9 \\
% {\color[HTML]{9B9B9B} Avion (ViT-B)~\cite{zhao2023training}}    & {\color[HTML]{9B9B9B} WIT + Ego4D}          & {\color[HTML]{9B9B9B} 49.1}   & {\color[HTML]{9B9B9B} 70.0} & {\color[HTML]{9B9B9B} 59.8} \\
% {\color[HTML]{9B9B9B} Avion (ViT-L)~\cite{zhao2023training}}    & {\color[HTML]{9B9B9B} WIT + Ego4D}          & {\color[HTML]{9B9B9B} \textbf{54.4}}   & {\color[HTML]{9B9B9B} 73.0} & {\color[HTML]{9B9B9B} \textbf{65.4}} \\

{Avion (ViT-B)~\cite{zhao2023training}}    & {WIT + Ego4D}          & { 49.1}   & { 70.0} & { 59.8} \\
{Avion (ViT-L)~\cite{zhao2023training}}    & { WIT + Ego4D}          & { \textbf{54.4}}   & { 73.0} & { \textbf{65.4}} \\
\midrule
Ours (ViT-B)              & None                 & 47.3      & 73.1    & 56.8    \\
Ours (ViT-B)             & Unlabeled K710                 & 47.0      & 73.0    & 56.3    \\
Ours (ViT-L)             & Unlabeled K710                 & 50.1      & \textbf{75.0}    & 59.5    \\
\bottomrule
\end{tabular}%
% }
\end{table}



==> tables/sota_d48.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{\textbf{Comparison to SOTA on Diving 48.}}
\label{tab:sota-d48}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Model         & Pre-train                 & Top-1 \\ \midrule
TimeSformer-L~\cite{bertasius2021space} & IN21K                     & 81.0  \\
VideoSwin-B~\cite{liu2022video}   & IN21K                     & 81.9  \\
BEVT~\cite{wang2022bevt}          & IN21K+K400                & 86.7  \\
SIFAR-B-14~\cite{fan2021can}    & IN21K                     & 87.3  \\
ORViT~\cite{herzig2022object}         & IN21K                     & 88.0  \\
AIM ViT-B/16~\cite{yang2023aim}  & CLIP                      & 88.9  \\
AIM ViT-L/14~\cite{yang2023aim}  & CLIP                      & 90.6  \\
MC-ViT-B~\cite{balavzevic2024memory}      & ALIGN+LTIP+JFT+HT100M+VTP & 89.7  \\
MC-ViT-L~\cite{balavzevic2024memory}      & ALIGN+LTIP+JFT+HT100M+VTP & 91.0  \\
Video-FocalNet-B~\cite{wasim2023video}      & K400 & 90.8  \\ \midrule
Ours (ViT-B)          & None                      & 87.8     \\
Ours (ViT-B)         & Unlabeled K710                      & 90.8     \\
Ours (ViT-L)          & Unlabeled K710                      & \textbf{93.\todo{X}}     \\
\bottomrule
\end{tabular}%
% }
\end{table}

==> tables/sota_ssv2.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Comparison to SOTA on Something-Something v2 \cite{goyal2017something}}}
\label{tab:sota-ssv2}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Model         & Pre-train                 & Top-1 \\ \midrule
PlaceHolder-L~\cite{bertasius2021space} & IN21K                     & 81.0  \\
Ours (ViT-B)         & K710                      & \todo{TBA}     \\
Ours (ViT-L)          & K710                      & \todo{TBA}     \\
\bottomrule
\end{tabular}%
% }
\end{table}

==> tables/unused_tables/long_video.tex <==


\begin{table}[]
\centering
\caption{\textbf{Dual masking enables training over long-video (128 frames)}. We find that (1) due to memory constraints there is no baseline with $100\%$ budget. (2) uniform decoder masking scheme such as ``Frame" performs outperforms random decoder masking which is consistent with \cite{wang2023videomae}. Lastly, (3) we obtain best results with our proposed Inverse-Forward dual masking scheme. \textit{Note that fine-tuning is performed using random-tube masking with $20\%$ and evaluation is reported on 1-crop}.}
\label{tab:long-video}
\begin{tabular}{@{}cccc|c@{}}
\toprule
   & \multicolumn{3}{c|}{MAE Pre-Training}    & Fine-Tuning        \\ \cmidrule(l){2-5} 
\# & Encoder Masking & Decoder Masking & $\rho_d$ & Noun-Verb Accuracy \\ \midrule
\texttt{1}  & Random Tube     & Random          & 33\%   & 43.3               \\
\texttt{2}  & Random Tube     & Frame           & 33\%   & 44.6               \\
\texttt{3}  & Inverse Flow    & Flow + Random   & 20\% + 10\%   & \textbf{44.8}               \\ \bottomrule
\end{tabular}
\end{table}


==> tables/unused_tables/short_video-old.tex <==


\begin{table}[]
\centering
\caption{\textbf{Dual masking strategies on short-video (32 frames)}. We find that (1) compared to no decoder mask (row \texttt{1}) with $100\%$ budget, uniform decoder masking scheme such as ``Frame" \cite{wang2023videomae} performs competitively with $1/3^{rd}$ (=$33\%$) token budget. With Forward decoder masking using Flow, we (2) observe better performance compared to baseline (row \texttt{3} vs. \texttt{1}), and lastly (3) we obtain best results with our proposed Inverse-Forward dual masking scheme (row \texttt{4}). \textit{Note that fine-tuning performance is reported on 1-crop}.}
\label{tab:short-video}
\begin{tabular}{@{}cccc|c@{}}
\toprule
   & \multicolumn{3}{c|}{MAE Pre-Training}    & Fine-Tuning        \\ \cmidrule(l){2-5} 
\# & Encoder Masking & Decoder Masking & $\rho_d$ & Noun-Verb Accuracy \\ \midrule
\texttt{1}  & Random Tube     & None            & 0\%    & 40.4               \\
\texttt{2}  & Random Tube     & Frame           & 33\%   & 40.1               \\
\texttt{3}  & Random Tube     & Flow + Random   & 20\% + 10\%   & 40.7               \\
\texttt{4}  & Inverse Flow    & Flow + Random   & 20\% + 10\%   & \textbf{40.8}               \\ \bottomrule
\end{tabular}
\end{table}

